Using Sustainability Impact Scores for Software Architecture Evaluation

For future regulatory compliance, organizations must assess and report on the state of sustainability in terms of its impacts over time. Sustainability, being a multidimensional concern, is complex to quantify. This complexity further increases with the interdependencies of the quality concerns across different sustainability dimensions. The research literature lacks a holistic way to evaluate sustainability at the software architecture level. With this study, our aim is to identify quality attribute (QA) trade-offs at the software architecture level and quantify the related sustainability impact. To this aim we present an improved version of the Sustainability Impact Score (SIS), building on our previous work. The SIS facilitates the identification and quantification of trade-offs in terms of their sustainability impact, leveraging a risk- and importance-based prioritization mechanism. To evaluate our approach, we apply it to an industrial case study involving a multi-model framework for integrated decision-making in the energy sector. Our study reveals that technical quality concerns have significant, often unrecognized impacts across sustainability dimensions. The SIS coupled with QA trade-offs can help practitioners make informed decisions that align with their sustainability goals. Early evaluations can help organizations mitigate sustainability risks by taking preventive actions.

==> comments.tex <==
\section{Intro}
% When it comes to SA evaluation, none of the existing approaches provide a mechanism to provide a quantitative sustainability impact assessment \cite{2023_Fatima_SLR}. Further, we see a lack of approaches looking at trade-offs in SA with a sustainability lens. 
% The evaluation of software architecture (SA) aims to ensure long-term quality. 
% \textbf{\textit{Are there any available solutions to perform sustainability assessment?}}
% \textbf{\textit{How do we build upon existing research to provide a solution?}}
% In this study, our aim is to provide a new version of the Sustainability Impact Score. To achieve this, we make changes across the following three steps of our SA Evaluation Method \cite{2024_Fatima_SA_Assessment_Method}. (i) \textit{Prioritization of Evaluation Criteria} -- through Risk and Importance based prioritization of QAs, (ii) \textit{Requirement Identification} -- by documenting the over-time sustainability impacts as part of the Sustainability Quality Model (SQ Model) \cite{Condori-Fernandez-2018-sqmodel}, and  (iii) \textit{Evaluation of obtained data} -- by providing a mechanism for relative comparison of SIS across different sustainability dimensions pairs (previously unsupported in \cite{2024_Fatima_SA_Assessment_Method}). 

% \textbf{\textit{Why is sustainability assessment relevant for the industry?}}

% We observe that conformance to interoperability requirements impacts the environment by the use of resources, benefit the society with accurate decision support and provides economic cost-effective solution for the public sector. A single architectural decisions can have a significant impact on the sustainability of and by this software, as both direct and systemic impacts. 

% However, none of the existing methods provide techniques for sustainability impact assessment across different sustainability dimensions (namely Economic, Environmental, Technical, Social \cite{Lago_2015-ssq}). \todo{mention MCDM methods and their limitations for sus assessment}


% In context of sustainability, \citet{Lago_2015-ssq} framed sustainability as a quality property and proposed using the sustainability quality requirements as an evaluation criteria. This idea is further elaborated in the SAF Toolkit \cite{} which explores the problem space for sustainability assessment through the use of decision maps, and use of dependency matrices to identify sustainability impacts. 


% In an ideal world, a quality attribute should improve based on its own definition. 

% We read the dependency matrix in such a way that all the quality attributes along the vertical axis are distributed. 

% \textit{Why do we need an architecture assessment?} 
% Think of your architecture as the structure of the human body. To maintain the health (quality) of the body over time, we need to take both preemptive and remedial steps. This requires a diagnosis (assessment) of the body to understand the current state of health and possible side effects of the treatment choices made. Similarly, to ensure the health of the software over time (sustainability), we need to diagnose the problems by assessing the conformance of architecture to the expected quality. Hence, the impacts of the architectural decisions must be analyzed to identify any side effects (or trade-offs). 

%%%%%% Contributions %%%%%%
% To this aim, we present a light-weight version of the architecture assessment approach for sustainability impact analysis. We improve upon our previous work \cite{2024_Fatima_SA_Assessment_Method} to develop an improved version of the sustainability impact score. We prioritize the quality of the system in terms of its importance and risk levels affecting the success of the project. 


% As SIS requires weights per QA rather than weights per scenario, we use the weight selection method used by \cite{S46}. In this method, if a criteria/sub-criteria inherits the weight of the associated scenario. If the criteria relates to more than one scenario, then its weight will be the maximum weight of the scenarios. 

% \subsection{From complexity to clarity}



% This priority can be calculated for each architectural alternative per scenario. SIS can consequently be utilized to support a decision-making process that considers sustainability.
% This scenario is contingent upon reducing resource utilization to ensure that there are no detrimental effects on performance, thereby harmonizing the benefits of resource utilization and performance.

% two architectural approaches (before and after) to analyze sustainability. Table \ref{tab:arch-approaches} shows the single model vs. multimodel approaches considered for this system. 
% We identify the issues associated with each option, the rationale for the support of an architectural approach and the evaluation criteria it will be evaluated on. 

\subsubsection{Inter-QA Trade-offs}
% The DMatrices show that there are no trade-offs between the QA sub-characteristics as we only focus on one QA \ie interoperability. We only observe QAs as having a positive impact or no impact on each other.  
% \subsubsection{Intra-QA trade-offs}
% Intra-QA trade-off refers to the tradeoff between the same QA defined differently as per the sustainabilty dimension. We observe intra QA trade-offs between different dimensions. For example, concurrency control leads to a negative impact on the economic dimension of sustainability in terms of cost of waiting time. As the execution times span over several hours, the workflows can remain in a waiting state for many hours to access a remote model. Although, this enables a smooth operation of the workflow across the technical dimension, it comes with an economic cost. 

\section{Discussion}
% With our current implementation, different QAs can have similar priority according to the % The paper is structured as follows. In Section \ref{sec:journeysofar}, we provide an overview of our previous approach. In Section \ref{sec:improvements}, we present the proposed improvements in SIS. In Section \ref{sec:case}, we provide an overview of the IT architecture that is used as a case study. In Section \ref{sec:methodology}, we provide an overview of the design of the case study using the approach proposed in Section \ref{sec:improvements}. In Section \ref{sec:results}, we provide the execution steps of the study and the results obtained. In Section \ref{sec:reflections}, we provide a discussion in terms of reflections and lessons learned.  In Section \ref{sec:relatedwork}, we provide an overview of the related work and our contribution to research using the presented approach. In Section \ref{sec:ttv} we discuss the threats to validity of our research and the applied mitigation steps. Finally, we provide a conclusion and future direction in Section \ref{sec:conclusion}. 
% The paper is structured as follows. In Section \ref{sec:journeysofar}, we provide an overview of our previous approach. In Section \ref{sec:improvements}, we present the proposed improvements in SIS. In Section \ref{sec:case}, we provide an overview of the IT architecture that is used as a case study. In Section \ref{sec:methodology}, we provide an overview of the design of the case study using the approach proposed in Section \ref{sec:improvements}. In Section \ref{sec:results}, we provide the execution steps of the study and the results obtained. In Section \ref{sec:reflections}, we provide a discussion in terms of reflections and lessons learned.  In Section \ref{sec:relatedwork}, we provide an overview of the related work and our contribution to research using the presented approach. In Section \ref{sec:ttv} we discuss the threats to validity of our research and the applied mitigation steps. Finally, we provide a conclusion and future direction in Section \ref{sec:conclusion}. 

% \textbf{A step towards sustainability monitoring.}

% In the context of our case study, we start with the interoperability concern as a challenge. Together with the study participant, we break down the interoperability into multiple QAs during the brainstorming process. To improve the evaluation process, breaking down QAs into sub-characteristics or associating them with measurable metrics can help clarify their relevance and make them more actionable. This decomposition enables the QAs to more accurately reflect the specific concerns they are trying to address in SA. In addition, these metrics can act as response measures in the scenario template provided by \citet{bass2012software}, which makes the success of the scenario measurable. In addition, linking these metrics with critical success factors using a KPI can help organizations monitor the improvement in sustainability overtime through continuous monitoring and analysis. \todo{cite a paper other than mine (:} Such an approach can be a step toward reporting sustainability for regulatory purposes in the future. 



% To apply MCDM methods like AHP, we need the same evaluation criteria on both sides of the matrix. However, with two sustainability dimensions represented in the DMatrix, the criteria could be similar, but also overlapping, or disjoint (see Fig.~\ref{fig:dmatrix-overview}).
% Hence, traditional MCDM methods like AHP cannot be applied in this case. 
% Related work shows that current methods lack an evaluation mechanism for sustainability impacts. MCDM approaches only work if the evaluation criteria are the same. However, in case of sustainability, the evaluation criteria can be the same but also overlapping or disjoint (see Fig.~\ref{fig:dmatrix-overview}), giving rise to rectangular matrices. To support these disjoint and overlapping criteria, our approach of using DMatrices together with the SIS helps identify the inter-QA trade-offs and impact on sustainability. 
% In addition, such methods have a tendency to increase the complexity of the evaluation for practitioners. 
% Our approach is based on the simple weighted sum method (WSM)~\cite{wiley_2021-gf} from the MCDM theory in combination with the DMatrix to create a SIS. We also provide reusable templates in our replication package \cite{rep-pkg}, which automates the quantification process. 

% The SIS provides a high-level overview of the trade-offs in terms of support for a certain sustainability dimension. 

% Furthermore, current MCDM methods do not meet the sustainability assessment needs due to the multidimensional nature of sustainability with overlapping criteria across dimensions. 

\section{Related Work}
\section{Introduction}


% START with reporting \cite{CSRD} -- organizations need to report sustainability -- need to improve it --- sustainability is multi dim -- to quantify impact -- we need a multi-dimensional index -- SIS provides it -- make better informed decisions -- by evaluating alternatives -- 

% now you can facilitate decision-making for sustainability - helps report on actual impacts and reporting improvements


% To solve this problem, we present an improved version of the Sustainability Impact Score (SIS), providing a high-level overview of sustainability support in terms of its impact. 

% One of the early definitions of sustainable development by \citet{Brundtland_1987} defines it as \textit{`meeting the needs of the present without compromising the ability of future generations to meet their own needs}. 

% In the context of digital ecosystems, ~\citet{Lago_ConnectedWorld_2023} defines sustainability as \textit{`the preservation of the beneficial use of digital solutions in a constantly changing context'}. This sustainability can be represented across various dimensions, such as economic (Ec), environmental (En), social (S), and technical (T)~\cite{Lago_2015-ssq}, with direct, enabling and systemic impacts~\cite{Hilty_2015}. 

% To ensure the sustainability of digital solutions, they must be evaluated early in the software lifecycle. 

% \changed{We observe that the current literature lacks in providing sustainability assessment approaches at the architecture level in a holistic way~\cite{2023_Fatima_SLR}.}
%
% We represent this priority in Eq.~\ref{eq:priority-score} as a function of importance and risk levels. 
% \begin{equation}
% \footnotesize
% \text{Priority}_{S_i} = \textit{$f (I , R) $}
% \label{eq:priority-score} %
% \end{equation}
% \text{\scriptsize $ S_i=\textit{ith Scenario}, I=\textit{Importance}, R = \textit{Risk}, I, R \in \{\text{High=3}, \text{Medium=2}, \text{Low=1}\} \; $}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% the architectural approach used for the MMvIB IT architecture. The approach aims to automate the process of running a multi model workflow and run single model processes based on the experiment setup. The choice of this approach is in line with the interoperability needs. In this study, we calculate the SIS for this approach and compare it to a theoretical optimal case. 

% We aim to identify measurable response measures of architectural scenarios and use them as indicators for sustainability monitoring in combination with the SIS. 
